On Random Subsampling of Gaussian Process Regression: A Graphon-Based Analysis

In this paper, we study random subsampling of Gaussian process regression, one of the simplest approximation baselines, from a theoretical perspective. Although subsampling discards a large part of training data, we show provable guarantees on the accuracy of the predictive mean/variance and its generalization ability. For analysis, we consider embedding kernel matrices into graphons, which encapsulate the difference of the sample size and enables us to evaluate the approximation and generalization errors in a unified manner. The experimental results show that the subsampling approximation achieves a better trade-off regarding accuracy and runtime than the Nystr\"{o}m and random Fourier expansion methods.

==> l2.tex <==
%!TEX root=./main.tex

\section{$\ell_2$ Norm}

\begin{lemma}[\cite{Levi:2018zz}]\label{lem:Levi}
  Let $\epsilon,L>0$ and let $A^1,\ldots,A^T \in [-L,L]^{n \times n}$ be matrices.
  Let $S \subseteq [n]$ be a set of $s = \Omega(\log n)$ elements uniformly and independently sampled from $[n]$.
  Then, with probability at least $0.99$, there exists a measure preserving bijection $\pi\colon[0,1]\to[0,1]$ such that, for every $t \in [T]$, we have
  \begin{align*}
    \|\mathcal{A}^t-\pi\left(\mathcal{A}^t_{S S}\right)\|_2 &\le O\left(L T\left(\epsilon + \sqrt{\frac{\log n}{s}} + \frac{1}{s^{1/4}}\left(\frac{1}{\epsilon}\right)^{O(T/\epsilon^2)}\right)\right).
  \end{align*}
\end{lemma}

\begin{theorem}\label{the:loss-l2}
  For any $\epsilon > 0$, Algorithm~\ref{alg:loss} with $s = \Theta(\log n) + (1/\epsilon)^{\Theta(1/\epsilon^2)}$ outputs $\widetilde{\bmalpha} \in \bbR^s$ such that
  \begin{align*}
    \ell_{K_{SS},\bmk_S,\lambda}(\widetilde{\bmalpha})
    = \ell_{K,\bmk,\lambda}(\bmalpha^*) \pm O\Bigl(\epsilon L^2 R^2 \Bigr)
  \end{align*}
  with probability at least $0.99$, where $\bmalpha^* = \argmin_{\bmalpha} \ell_{K,\bmk,\lambda}(\bmalpha)$, $L = \max\set{\|K\|_{\max},\|\bmk\|_\infty}$, and $R = \max\set{\|\bmalpha^*\|_2/\sqrt{n},\|\widetilde{\bmalpha}\|_2/\sqrt{s} }$.
\end{theorem}


Now, we show that minimizing $\ell_{K,\bmk,\lambda}$ and $\ell_{\calK,\calk,\lambda}$ are equivalent:
\begin{lemma}\label{lem:equivalence-l2}
  For any $R \in \bbR_+$, we have
  \begin{align*}
    \min_{\bmalpha \in \bbR^n:\|\bmalpha\|_2 \leq \sqrt{n}R} \ell_{K,\bmk,\lambda}(\bmalpha)
    =
    \min_{f: [0,1] \to \bbR:\|f\|_2 \leq R} \ell_{\calK,\calk,\lambda}(f)
  \end{align*}
\end{lemma}
\begin{proof}
  First, we show (RHS) $\leq$ (LHS).
  Let $\bmalpha^*$ be a minimizer of the LHS and let $f\colon[0,1] \to \bbR$ with $f(x) = \alpha^*_{i_n(x)}$.
  Note that $\|f\|_2 = \|\bmalpha^*\|_2/\sqrt{n}$.
  As $f$ is $n$-block constant, by Lemma~\ref{lem:block-constant}, we have $\ell_{\calK,\calk,\lambda}(f) = \ell_{K,\bmk,\lambda}(\bmalpha^*)$.

  Next, we show (LHS) $\leq$ (RHS).
  Let $f^*:[0,1]\to \bbR$ be a minimizer of the RHS. \ynote{it could be there's no minimizer.}
  First, we observe that we can assume $f(x)=f(x')$ for every $x,x'\in [0,1]$ with $i_n(x)=i_n(x')$.
  To see this, note that $\ell_{\calK,\calk,\lambda}$ is convex and is invariant under swapping $f(x)$ and $f(x')$ for any $x,x'\in [0,1]$ with $i_n(x)=i_n(x')$.
  Hence, we can decrease the value of $\ell_{\calK,\calk,\lambda}$ by taking the average of $f(x)$ and $f(x')$.
  Moreover, $\|f\|_2$ does not increase through this modification.
  This means that there is a minimizer $f^*$ of $\ell_{\calK,\calk,\lambda}$ with the desired property.
  Now as $f^*$ is $n$-block constant, Lemma~\ref{lem:block-constant} gives a vector $\bmalpha \in \bbR^n$ such that $\ell_{K,\bmk,\lambda}(\bmalpha) \leq \ell_{\calK,\calk,\lambda}(f^*)$.
  Also, $\|\bmalpha\|_2/\sqrt{n} = \|f^*\|$.
\end{proof}



\begin{lemma}\label{lem:subsampling-l2}
  If a set $S \subseteq [n]$ satisfies
  \[
    \|\calK - \pi(\calK_{SS})\|_2 \leq \epsilon L \text{ and } \|\calk - \pi(\calk_S)\|_2 \leq \epsilon L
  \]
  for some measure-preserving bijection $\pi\colon[0,1]\to[0,1]$, then we have
  \[
    \min_{\widetilde{\bmalpha} \in \bbR^s} \ell_{K_{SS},\bmk_S,\lambda}(\widetilde{\bmalpha})
    =
    \min_{\bmalpha \in \bbR^n} \ell_{K,\bmk,\lambda}(\bmalpha)   \pm O\Bigl(\epsilon L^2 R^2 \Bigr)
  \]
\end{lemma}
\begin{proof}
  We have
  \begin{align*}
    & \min_{\bmalpha \in \bbR^s} \ell_{K_{SS},\bmk_S,\lambda}(\bmalpha) = \min_{\bmalpha \in \bbR^s:\|\bmalpha\|_2 \leq \sqrt{s}R} \ell_{K_{SS},\bmk_S,\lambda}(\bmalpha) \\
    & =
    \min_{\bmalpha \in \bbR^s\colon \|\bmalpha\|_2 \leq \sqrt{s}R} \frac{1}{s^3}\|K_{SS}\bmalpha\|_2^2- \frac{2}{s^2} \langle \bmk_S, K_{SS}\bmalpha\rangle + \frac{1}{s}\|\bmk_S\|_2^2  + \frac{\lambda}{n^2} \langle \bmalpha, K_{SS} \bmalpha\rangle \\
    & =
    \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}} \| \calK_{SS} f\|_2^2- 2 \langle \calk_S, \calK_{SS} f \rangle + \|\calk_S\|_2^2 + \lambda \langle f, \calK_{SS} f\rangle \tag{By Lemma~\ref{lem:equivalence-l2}}\\
    & = \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}} \| \pi(\calK_{SS}) f\|_2^2- 2 \langle \pi(\calk_S), \pi(\calK_{SS}) f \rangle + \|\pi(\calk_S)\|_2^2 + \lambda \langle f, \pi(\calK_{SS}) f\rangle \\
    & =
    \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}} \| (\pi(\calK_{SS})-\calK+\calK) f\|_2^2- 2 \langle \pi(\calk_S) - \calk + \calk, (\pi(\calK_{SS}) - \calK + \calK)f \rangle   \\
    & \qquad \qquad \qquad + \|\pi(\calk_S) - \calk + \calk\|_2^2 + \lambda  \langle f, (\pi(\calK_{SS}) -\calK+\calK) f\rangle\\
    & =
    \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}} \|\calK f\|_2^2  + 2\langle (\pi(\calK_{SS})-\calK) f, \calK f \rangle  + \| (\pi(\calK_{SS})-\calK) f\|_2^2   \\
    &\qquad \qquad\qquad - 2 \langle \calk, \calK f \rangle - 2 \langle \calk, (\pi(\calK_{SS}) - \calK)f \rangle - 2 \langle \pi(\calk_S)-\calk, \calK f \rangle - 2 \langle \pi(\calk_S) - \calk, (\pi(\calK_{SS}) - \calK)f \rangle\\
    & \qquad \qquad\qquad +  \|\calk\|_2^2 + 2\langle \pi(\calk_S)-\calk,\calk\rangle + \|\pi(\calk_S)-\calk\|_2^2  \\
    & \qquad \qquad\qquad + \lambda  \langle f, \calK f\rangle + \lambda  \langle f, (\pi(\calK_{SS})- \calK) f\rangle
  \end{align*}
  By Cauchy-Schwarz, we have
  \begin{align*}
    & =
    \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}}  \|\calK f\|_2^2 - 2 \langle \calk, \calK f \rangle + \|\calk\|_2^2 + \lambda  \langle f, \calK f\rangle  \\
    &\qquad \qquad\qquad \pm \Bigl(2 \|\pi(\calK_{SS})-\calK\|_2 \|\calK\|_2 \|f\|_2^2  +  \|\pi(\calK_{SS})-\calK\|_2^2 \|f\|_2^2  \\
    & \qquad \qquad\qquad \qquad + 2 \|\pi(\calK_{SS}) - \calK\|_2 \|\calk\|_2 \|f\|_2 + 2 \|\calK\|_2 \|\pi(\calk_S)-\calk\|_2 \|f\|_2 \\
    & \qquad \qquad\qquad \qquad + 2 \|\pi(\calK_{SS}) - \calK\|_2 \|\pi(\calk_S)- \calk\|_2 \|f\|_2 + 2\|\pi(\calk_S)-\calk\|_2\|\calk\|_2  \\
    & \qquad \qquad\qquad \qquad  + \|\pi(\calk)-\calk\|_2^2 + \lambda \|\pi(\calK_{SS})-\calK\|_2\|f\|_2^2 \Bigr)
  \end{align*}
  From the assumption, we have
  \begin{align*}
    & =
    \min_{\substack{f\colon [0,1] \to \bbR: \\ \|f\|_2 \leq R}} \|\calK f\|_2^2 - 2 \langle \calk, \calK f \rangle + \|\calk\|_2^2 + \lambda \langle f, \calK f\rangle  \\
    &\qquad \qquad\qquad \pm \Bigl(2 \epsilon L^2 R^2  + \epsilon^2 L^2  R^2 + 2 \epsilon L^2 R + 2 \epsilon L^2 R + 2 \epsilon^2 L^2 R + 2\epsilon L^2 + \epsilon^2 L^2 + \lambda \epsilon L R^2\Bigr) \\
    & = \min_{\bmalpha \in \bbR^n : \|\bmalpha\|_2 \leq \sqrt{n}R} \frac{1}{n^3} \|K \bmalpha\|_2^2 - \frac{2}{n^2} \langle \bmk, K \bmalpha \rangle + \frac{1}{n}\|\bmk\|_2^2 + \frac{\lambda}{n^2} \langle \bmalpha, \calK \bmalpha \rangle \pm O\Bigl( \epsilon L^2 R^2\Bigr) \tag{By Lemma~\ref{lem:equivalence-l2}} \\
    & = \min_{\bmalpha \in \bbR^n : \|\bmalpha\|_2 \leq \sqrt{n}R} \ell_{K,\bmk,\lambda}(\bmalpha)  \pm O\Bigl(\epsilon L^2 R^2 \Bigr) \\
    & = \min_{\bmalpha \in \bbR^n } \ell_{K,\bmk,\lambda}(\bmalpha)  \pm O\Bigl(\epsilon L^2 R^2 \Bigr)
  \end{align*}
  as desired.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{the:loss-l2}]
  By Lemma~\ref{lem:Levi} on $K$ and $\bmk \bmone^\top$, we have
  \[
    \|\calK - \pi(\calK_{SS})\|_2 \leq \epsilon L \text{ and } \|\calk - \pi(\calk_S)\|_2 \leq \epsilon L.
  \]
  holds for some measure-preserving bijection $\pi\colon[0,1]\to[0,1]$   with probability at least 0.99.
  Then, the theorem follows by Lemma~\ref{lem:subsampling-l2}.
\end{proof}


\begin{lemma}\label{lem:subsampling-l2-with-solution}
  If a set $S \subseteq [n]$ satisfies
  \[
    \|\calK - \pi(\calK_{SS})\|_2 \leq \epsilon L \text{ and } \|\calk - \pi(\calk_S)\|_2 \leq \epsilon L
  \]
  for some measure-preserving bijection $\pi\colon[0,1]\to[0,1]$, then for any $\widetilde{\bmalpha} \in \bbR^s$ with $\|\widetilde{\bmalpha}\|_2 \leq \sqrt{s}R$, there exists $\bmalpha \in \bbR^n$ such that
  \[
    \ell_{K_{SS},\bmk_S,\lambda}(\widetilde{\bmalpha})
    =
    \ell_{K,\bmk,\lambda}(\bmalpha) \pm O\Bigl(\epsilon L^2 R^2 \Bigr).
  \]
  Moreover, we have $\pi(f_{\widetilde{\bmalpha}}) = f_{\bmalpha}$.
\end{lemma}
\begin{proof}
  We have
  \begin{align*}
    & \ell_{K_{SS},\bmk_S,\lambda}(\widetilde{\bmalpha}) \\
    & =
    \frac{1}{s^3}\|K_{SS}\widetilde{\bmalpha}\|_2^2- \frac{2}{s^2} \langle \bmk_S, K_{SS}\widetilde{\bmalpha}\rangle + \frac{1}{s}\|\bmk_S\|_2^2  + \frac{\lambda}{n^2} \langle \widetilde{\bmalpha}, K_{SS} \widetilde{\bmalpha}\rangle \\
    & =
    \| \calK_{SS} \widetilde{f}\|_2^2- 2 \langle \calk_S, \calK_{SS} \widetilde{f} \rangle + \|\calk_S\|_2^2 + \lambda \langle \widetilde{f}, \calK_{SS} \widetilde{f}\rangle \tag{By Lemma~\ref{lem:block-constant}}\\
    & = \| \pi(\calK_{SS}) \pi(\widetilde{f})\|_2^2- 2 \langle \pi(\calk_S), \pi(\calK_{SS}) \pi(\widetilde{f}) \rangle + \|\pi(\calk_S)\|_2^2 + \lambda \langle \pi(\widetilde{f}), \pi(\calK_{SS}) \pi(\widetilde{f})\rangle \\
    & =
    (\pi(\calK_{SS})-\calK+\calK) \pi(\widetilde{f})\|_2^2- 2 \langle \pi(\calk_S) - \calk + \calk, (\pi(\calK_{SS}) - \calK + \calK)\pi(\widetilde{f}) \rangle   \\
    & \qquad \qquad \qquad + \|\pi(\calk_S) - \calk + \calk\|_2^2 + \lambda  \langle \pi(\widetilde{f}), (\pi(\calK_{SS}) -\calK+\calK) \pi(\widetilde{f})\rangle\\
    & =
    \|\calK \pi(\widetilde{f})\|_2^2  + 2\langle (\pi(\calK_{SS})-\calK) \pi(\widetilde{f}), \calK \pi(\widetilde{f}) \rangle  + \| (\pi(\calK_{SS})-\calK) \pi(\widetilde{f})\|_2^2   \\
    &\qquad \qquad\qquad - 2 \langle \calk, \calK \pi(\widetilde{f}) \rangle - 2 \langle \calk, (\pi(\calK_{SS}) - \calK)\pi(\widetilde{f}) \rangle - 2 \langle \pi(\calk_S)-\calk, \calK \pi(\widetilde{f}) \rangle - 2 \langle \pi(\calk_S) - \calk, (\pi(\calK_{SS}) - \calK)\pi(\widetilde{f}) \rangle\\
    & \qquad \qquad\qquad +  \|\calk\|_2^2 + 2\langle \pi(\calk_S)-\calk,\calk\rangle + \|\pi(\calk_S)-\calk\|_2^2  \\
    & \qquad \qquad\qquad + \lambda  \langle \pi(\widetilde{f}), \calK \pi(\widetilde{f})\rangle + \lambda  \langle \pi(\widetilde{f}), (\pi(\calK_{SS})- \calK) \pi(\widetilde{f})\rangle
  \end{align*}
  By Cauchy-Schwarz, we have
  \begin{align*}
    & =
    \|\calK \pi(\widetilde{f})\|_2^2 - 2 \langle \calk, \calK \pi(\widetilde{f}) \rangle + \|\calk\|_2^2 + \lambda  \langle \pi(\widetilde{f}), \calK \pi(\widetilde{f})\rangle  \\
    &\qquad \qquad\qquad \pm \Bigl(2 \|\pi(\calK_{SS})-\calK\|_2 \|\calK\|_2 \|\pi(\widetilde{f})\|_2^2  +  \|\pi(\calK_{SS})-\calK\|_2^2 \|\pi(\widetilde{f})\|_2^2  \\
    & \qquad \qquad\qquad \qquad + 2 \|\pi(\calK_{SS}) - \calK\|_2 \|\calk\|_2 \|\pi(\widetilde{f})\|_2 + 2 \|\calK\|_2 \|\pi(\calk_S)-\calk\|_2 \|\pi(\widetilde{f})\|_2 \\
    & \qquad \qquad\qquad \qquad + 2 \|\pi(\calK_{SS}) - \calK\|_2 \|\pi(\calk_S)- \calk\|_2 \|\pi(\widetilde{f})\|_2 + 2\|\pi(\calk_S)-\calk\|_2\|\calk\|_2  \\
    & \qquad \qquad\qquad \qquad  + \|\pi(\calk)-\calk\|_2^2 + \lambda \|\pi(\calK_{SS})-\calK\|_2\|\pi(\widetilde{f})\|_2^2 \Bigr)
  \end{align*}
  From the assumption, we have
  \begin{align*}
    & =
    \|\calK \pi(\widetilde{f})\|_2^2 - 2 \langle \calk, \calK \pi(\widetilde{f}) \rangle + \|\calk\|_2^2 + \lambda \langle \pi(\widetilde{f}), \calK \pi(\widetilde{f})\rangle  \\
    &\qquad \qquad\qquad \pm \Bigl(2 \epsilon L^2 R^2  + \epsilon^2 L^2  R^2 + 2 \epsilon L^2 R + 2 \epsilon L^2 R + 2 \epsilon^2 L^2 R + 2\epsilon L^2 + \epsilon^2 L^2 + \lambda \epsilon L R^2\Bigr) \\
    & = \frac{1}{n^3} \|K \bmalpha\|_2^2 - \frac{2}{n^2} \langle \bmk, K \bmalpha \rangle + \frac{1}{n}\|\bmk\|_2^2 + \frac{\lambda}{n^2} \langle \bmalpha, \calK \bmalpha \rangle \pm O\Bigl( \epsilon L^2 R^2\Bigr) \tag{By Lemma~\ref{lem:equivalence-l2}} \\
    & = \ell_{K,\bmk,\lambda}(\bmalpha)  \pm O\Bigl(\epsilon L^2 R^2 \Bigr).
  \end{align*}
  as desired.
\end{proof}

==> tbl/prediction.tex <==
\begin{tabular}{lrrrrr}
  \toprule
Method & abalone & cpusmall & housing & mg & space\_ga \\
  \midrule
Proposed $s=20$ & 0.6009 & 0.6811 & 0.5743 & 0.4821 & 0.9523 \\
  Proposed $s=40$ & 0.6542 & 0.6129 & 0.3364 & 0.4420 & 0.8079 \\
  Proposed $s=80$ & 0.4959 & 0.1754 & 0.3341 & 0.3599 & 0.5565 \\
  Baseline & 0.4701 & 0.0551 & 0.2978 & 0.2733 & 0.4726 \\
   \bottomrule
\end{tabular}


==> variance.tex <==
%!TEX root=./main.tex

\section{Computing Predictive Variance}\label{sec:variance}

In this section, we give a method for computing predictive variance in \ref{def:pred} and investigate its performance.
For brevity, we introduce the following notation for the second term of the predictive variance as
\begin{align*}
	\zeta(\bmx^*) := \bmk_{\bmx^*}^\top (K+\lambda  I)^{-1} \bmk_{\bmx^*}.
\end{align*}


Using $K_{SJ}$ and $K_{JJ}$, we propose an approximate method for $\zeta(\bmx^*)$ as
\begin{align}
	\hat{\zeta}(\bmx^*) & = \bmk_{\bmx^*}^T (K_{SJ}^\top K_{SJ} + \lambda K_{JJ})^{\dagger}\bmk_{\bmx^*},
\end{align}
where $H^\dagger$ denotes a Moore-Penrose inverse of a matrix $H$.

%\begin{align*}
%  \tilde{\sigma}^2(x) & =\eta^2 \bmk_\bmx^T (H^\top H + \eta^2 \widetilde{K})^{-1}\bmk_\bmx, \\
%  \check{\sigma}^2(x) & =\eta^2 \bmk_\bmx^T (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}\bmk_\bmx.
%\end{align*}
%\ynote{Can we assume the inverses exist?}

We bound an approximation error for the variance of posterior distributions.

\begin{theorem}
  For any $\delta > 0$, we have
  \begin{align*}
    |\tilde{\sigma}^2(x) - \check{\sigma}^2(x)| \leq \eta^2 \left(2 \log \frac{2}{\delta} \left(\frac{m+s}{ms} \right) + \sqrt{2 \log \frac{2}{\delta} \left(\frac{m+s}{ms} \right)} \right)
  \end{align*}
  with probability at least $1-2\delta$. \ynote{what's the randomness here?}
\end{theorem}
\begin{proof}
  We have
  \begin{align*}
    &\tilde{\sigma}^2(x) - \check{\sigma}^2(x)\\
    &=\eta^2 \bmk_\bmx^T (H^\top H + \eta^2 \widetilde{K})^{-1}\bmk_\bmx - \eta^2 \bmk_\bmx^T (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}\bmk_\bmx\\
    &=\eta^2 \bmk_\bmx^T \left((H^\top H + \eta^2 \widetilde{K})^{-1} - (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}\right)\bmk_\bmx.
  \end{align*}
  The term in the large parentheses can be rephrased as
  \begin{align*}
    &(H^\top H + \eta^2 \widetilde{K})^{-1} - (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}\\
    &=(\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}(\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})(H^\top H + \eta^2 \widetilde{K})^{-1} - (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1}\\
    &=(\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1} \left((\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})(H^\top H + \eta^2 \widetilde{K})^{-1} - (H^\top H + \eta^2 \widetilde{K})(H^\top H + \eta^2 \widetilde{K})^{-1} \right)\\
    &= (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1} (\widetilde{H}^\top \widetilde{H} - H^\top H ) (H^\top H + \eta^2 \widetilde{K})^{-1},
  \end{align*}
  which yields
  \begin{align}
    &\tilde{\sigma}^2(x) - \check{\sigma}^2(x)=\eta^2 \bmk_\bmx^T (\widetilde{H}^\top \widetilde{H} + \eta^2 \widetilde{K})^{-1} (\widetilde{H}^\top \widetilde{H} - H^\top H ) (H^\top H + \eta^2 \widetilde{K})^{-1}\bmk_\bmx. \label{rep:dif}
  \end{align}

  We introduce an operator $Z_m\colon f \mapsto (\langle K(\cdot,\bmx_1),f\rangle ,\ldots,\langle K(\cdot,\bmx_m), f \rangle)$ \ynote{Do you really want to use $\bmx_1,\ldots,\bmx_m$ instead of $\set{\bmx_j \mid j \in J}$?} \ynote{What's the type of $f$?} and let $Z_m^*$ be its adjoint operator.
  Let $C_n$ be a covariance operator such that $\langle f, C_n f' \rangle = n^{-1}\sum_{i \in [n]} f(\bmx_i)f'(\bmx_i)$.
  Define $C_m$ and $C_s$ analogously.
  Let $Z_m = U \Sigma V^*$ be the singular value decomposition of $Z_m$, where $\Sigma \in \bbR^{t \times t}$ is a diagonal matrix with positive diagonal elements.

  Applying Lemmas~2 and~3 in~\cite{rudi2015less}, we can rewrite~\eqref{rep:dif} as
  \begin{align}
    \tilde{\sigma}^2(x) - \check{\sigma}^2(x)&=\eta^2 V (V^* C_s V + \lambda I)^{-1} V^* (C_s - C_n) V  (V^* C_n V + \lambda I)^{-1}V^* \notag \\
    &=g(C_s) (C_s - C_n) g(C_n), \label{rep:dif2}
  \end{align}
  where $g(C):=V (V^* C V + \lambda I)^{-1} V^*$.
  Then, we can bound~\eqref{rep:dif2} as
  \begin{align*}
    &|g(C_s) (C_s - C_n) g(C_n)| \leq \beta^2 \|C_s - C_n\|  \leq  \beta^2 \left( \frac{1}{s} \sum_{i \in [s]} h(\bmx_i) - \frac{1}{n} \sum_{i' \in [n]} h(\bmx_{i'}) \right),
  \end{align*}
  where $h(\bmx)$ is an existing function formed by orthonormal functions (*) \ynote{what does this mean?} and $\beta > 0$ is defined as in Theorem~1 in~\cite{rudi2015less}.
  Then, using concentration inequalities (e.g. Proposition 1.1 in \cite{rudi2015less}), we obtain
  \begin{align*}
    \left| \frac{1}{s} \sum_{i \in [s]} h(\bmx_i) - \frac{1}{n} \sum_{i' \in [n]} h(\bmx_{i'}) \right| \leq \frac{2 \log \frac{2}{\delta}}{m} + \sqrt{\frac{2 \log \frac{2}{\delta}}{m}} + \frac{2 \log \frac{2}{\delta}}{s} + \sqrt{\frac{2 \log \frac{2}{\delta}}{s}},
  \end{align*}
  with probability at least $1-2\delta$.
\end{proof}
